Combination of the W boson polarization measurements in top quark decays using ATLAS and CMS data at $\sqrt{s} =$ 8 TeV

The combination of measurements of the W boson polarization in top quark decays performed by the ATLAS and CMS Collaborations is presented. The measurements are based on proton-proton collision data produced at the LHC at a centre-of-mass energy of 8 TeV, and corresponding to an integrated luminosity of about 20 fb$^{-1}$ for each experiment. The measurements used events containing one lepton and having different jet multiplicities in the final state. The results are quoted as fractions of W bosons with longitudinal ($F_0$), left-handed ($F_\mathrm{L}$), or right-handed ($F_\mathrm{R}$) polarizations. The resulting combined measurements of the polarization fractions are $F_0 =$ 0.693 $\pm$ 0.014 and $F_\mathrm{L} =$ 0.315 $\pm$ 0.011. The fraction $F_\mathrm{R}$ is calculated from the unitarity constraint to be $F_\mathrm{R} = -$0.008 $\pm$ 0.007. These results are in agreement with the standard model predictions at next-to-next-to-leading order in perturbative quantum chromodynamics and represent an improvement in precision of 25 (29)% for $F_0$ ($F_\mathrm{L}$) with respect to the most precise single measurement. A limit on anomalous right-handed vector ($V_{\text{R}}$), and left- and right-handed tensor ($g_{\text{L}},g_{\text{R}}$) tWb couplings is set while fixing all others to their standard model values. The allowed regions are [$-$0.11, 0.16] for $V_{\text{R}}$, [$-$0.08, 0.05] for $g_{\text{L}}$, and [$-$0.04, 0.02] for $g_{\text{R}}$, at 95% confidence level. Limits on the corresponding Wilson coefficients are also derived.

==> Comb_method.tex <==
\section{Combination method}
\label{sec:method}

The combination is performed by finding the best linear unbiased estimator (BLUE)~\cite{Lyons:1988rp,Valassi:2003mu}. The BLUE method finds the coefficients of the linear combination of the input measurements by minimising the total uncertainty of the combined result, taking into account both the statistical and systematic uncertainties, as well as correlations between the inputs.

Imposing a unitarity constraint between the three observables, \FZ, \FL , and \FR, results in two independent observables. In this analysis, the measurements of \FZ\ and \FL\ are combined while \FR\ is obtained as \mbox{$\FR = 1-\FZ-\FL$}. As no further  constraint on the observables was placed, values outside the range [0,1] are allowed for the three polarisation fractions. %The uncertainty on \FR~ is estimated considering the total correlation between \FZ\ and \FL\ provided by BLUE.
The  total correlation between \FZ\ and \FL\ obtained from the combination is taken into account in the estimation of the uncertainty on the \FR~value.

%Since two observables, \FZ\ and \FL, are measured in the present analysis, each measurement comes with two weights, the \emph{BLUE coefficients}, for the overall LHC combination presented in Section~\ref{sec:results}.

%The implemented combination method takes into account the statistical and systematic uncertainties including correlations between the measured polarisation fractions in each systematic uncertainty category as well as the correlations among the measurements.

%As the BLUE algorithm accepts only symmetric uncertainties, the uncertainties of the ATLAS measurement are symmetrised by assigning the average uncertainty value between the up and down variations in each uncertainty source. A test has been performed by replacing the average uncertainty value with the largest shift among the up and down variations. The change in the combination results was observed to be negligible. In addition, common uncertainty categories are established by merging and regrouping various uncertainties in each individual input measurement. See Section~\ref{sec:systematics} and~\ref{sec:correlation} for more details.
%-----------------------------------------------------------

